Revisiting Chain-of-Thought Reasoning under Limited Supervision: Semi-supervised Chain-of-Thought Learning

Chain-of-thought (CoT) reasoning has emerged as an effective approach for activating latent reasoning capabilities in large language models. However, most existing CoT methods use reasoning chains mainly as inference-time prompts, while the generated reasoning traces are rarely reused as semi-supervised learning signals. In this report, we define \textbf{Semi-supervised Chain-of-Thought Learning} and propose \textbf{Semi-CoT}, a simple framework that uses unlabeled questions to construct pseudo reasoning supervision. Semi-CoT samples multiple pseudo-CoTs for each unlabeled question, estimates answer-level semantic entropy, and selects low-entropy reasoning chains as reliable pseudo-CoT demonstrations. This extends the self-training view of CoT from inference-time refinement to semi-supervised pseudo-supervision. Pilot experiments on AQuA, SVAMP, GSM8K, and MultiArith show that the entropy gate selects high-precision pseudo-CoTs, with pseudo-answer precision ranging from $91.36\%$ to $100\%$. Semi-CoT also gives small gains on SVAMP and GSM8K, while AQuA shows negative transfer and MultiArith reaches a ceiling. These results suggest that unlabeled questions can provide reliable pseudo reasoning signals, but their effective use still requires stronger demonstration selection or student training.

==> sections/tables/Real_world_results.tex <==
\begin{table}[t]
    \begin{minipage}{0.35\linewidth}
        \centering
        \setlength{\lineskip}{1pt} 
        \includegraphics[width=\linewidth]{sections/figures/real_vis.pdf}
        \captionof{figure}{\textbf{Visualization of real-world setup.} Top: Physical corruptions (Oil and Shelter). Bottom: Initial states of four evaluation tasks.}
        \label{fig:vis_real}
    \end{minipage}
    \hfill
    % \centering
    \begin{minipage}{0.63\linewidth}
        \centering
        \caption{\textbf{Real-world robustness evaluation.} ``\textbf{Clean}'' reports the absolute success rate (\%). All other columns report the \textbf{performance change} (percentage points, $\Delta$) relative to the clean setting. \textbf{Noise} and \textbf{Blur} represent the average performance drop across different severity levels. \textit{\textbf{Oil}} and \textit{\textbf{Shelter}} denote physical interferences. \textbf{Bold} indicates the best robustness (smallest performance drop).}
        \label{tab:main_results}
        \begin{small}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{ll|c|cccc|c}
            \toprule
            \textbf{Task} & \textbf{Method} & \textbf{Clean} & \textbf{Noise} ($\Delta$) & \textbf{Blur} ($\Delta$) & \textbf{\textit{Oil}} ($\Delta$) & \textbf{\textit{Shelter}} ($\Delta$) & \textbf{Avg.} ($\Delta$) \\
            \midrule

            \multirow{3}{*}{\makecell[l]{Pick\\and place}} 
            & $\pi_{0.5}$        & 100.0 & -63.3 & -16.7 & -10.0 & -30.0 & -30.1 \\
            & VLA-Adapter        & 80.0  & -66.7 & -40.0 & -30.0 & -60.0 & -49.2 \\
            & \textbf{StableVLA} & 80.0  & \textbf{-30.0} & \textbf{-10.0} & \textbf{-10.0} & \textbf{-20.0} & \textbf{-17.5} \\
            \midrule

            \multirow{3}{*}{\makecell[l]{Throw\\basketball}}
            & $\pi_{0.5}$        & 80.0 & -60.0 & -33.3 & -20.0 & -30.0 & -35.8 \\
            & VLA-Adapter        & 60.0 & -53.0 & -40.0 & -20.0 & -40.0 & -38.3 \\
            & \textbf{StableVLA} & 60.0 & \textbf{-36.7} & \textbf{-16.7} & \textbf{-10.0} & \textbf{-10.0} & \textbf{-18.4} \\
            \midrule

            \multirow{3}{*}{Pour water}
            & $\pi_{0.5}$        & 70.0 & -60.0 & -20.0 & -20.0 & -20.0 & -30.0 \\
            & VLA-Adapter        & 40.0 & -40.0 & -30.0 & -10.0 & -20.0 & -25.0 \\
            & \textbf{StableVLA} & 40.0 & \textbf{-23.3} & \textbf{-16.7} & \textbf{-0.0} & \textbf{-10.0} & \textbf{-12.5} \\
            \midrule

            \multirow{3}{*}{Pack doll}
            & $\pi_{0.5}$        & 80.0 & -63.3 & -33.3 & -30.0 & -40.0 & -41.7 \\
            & VLA-Adapter        & 50.0 & -40.0 & -26.7 & -30.0 & -30.0 & -31.7 \\
            & \textbf{StableVLA} & 60.0 & \textbf{-16.7} & \textbf{-10.0} & \textbf{-20.0} & \textbf{-10.0} & \textbf{-14.2} \\

            \bottomrule
            \label{tab:real_res}
            \end{tabular}
        }
        \end{small}
    \end{minipage}
\vspace{-10pt}
\end{table}


==> sections/tables/compare_base.tex <==
% % Table 1: Summary comparison on LIBERO benchmark
% % Auto-generated from CSV data
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{4pt}
% \caption{Performance and runtime comparison between StableVLA and other baselines on LIBERO benchmark under different levels of visual corruptions. We report the averaged success rate (\%) and the averaged inference runtime across 4 task suites. Results under each corruption level are averaged over all corruption types. The best results are highlighted in \textbf{bold} and the second best is highlighted in \underline{underline}.}
% \label{tab:efficiency-landscape}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% Method & \makecell{Param.\\(B)} & \makecell{Infer\\time (s)}&  Clean & Sev 3 & Sev 4 & Sev 5 & Avg \\
% \midrule
% OpenVLA & 7 & & 69.8 & 29.6 & 18.6 & 10.2 & 19.5 \\
% OpenVLA-OFT & 7 & & 95.5 & 86.0 & 74.9 & 58.9 & 73.3 \\
% OpenPI & 3 & &\textbf{96.8} & \underline{87.2} & \underline{78.9} & \underline{62.7} & \underline{76.2} \\
% VLA-Adapter & 0.5 & & 96.2 & 76.9 & 58.3 & 40.3 & 58.5 \\
% StableVLA & 0.5 & & \underline{96.7} & \textbf{89.1} & \textbf{80.8} & \textbf{67.4} & \textbf{79.1} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
% Table 1: Summary comparison on LIBERO benchmark
% Auto-generated from CSV data
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{4pt}
% \caption{Performance and runtime comparison between StableVLA and other baselines on LIBERO benchmark under different levels of visual corruptions. We report the averaged success rate (\%) and the averaged inference runtime across 4 task suites. Results under each corruption level are averaged over all corruption types. The best results are highlighted in \textbf{bold} and the second best is highlighted in \underline{underline}.}
% \label{tab:efficiency-landscape}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
% Method & \makecell{Param.\\(B)} &  Clean & Sev 3 & Sev 4 & Sev 5 & Avg \\
% \midrule
% OpenVLA & 7 & 69.8 & 29.6 & 18.6 & 10.2 & 19.5 \\
% OpenVLA-OFT & 7 & 95.5 & 86.0 & 74.9 & 58.9 & 73.3 \\
% OpenPI & 3 &\textbf{96.8} & \underline{87.2} & \underline{78.9} & \underline{62.7} & \underline{76.2} \\
% VLA-Adapter & 0.5 & 96.2 & 76.9 & 58.3 & 40.3 & 58.5 \\
% StableVLA & 0.5 & \underline{96.7} & \textbf{89.1} & \textbf{80.8} & \textbf{67.4} & \textbf{79.1} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
\begin{figure}[htbp]
\centering
\begin{subfigure}[c]{0.42\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sections/figures/radar_4tasks_with_clean.pdf}
    \caption{Robustness comparison across corruption types on LIBERO. See Appendix~\ref{app:radar} for details.}
    \label{fig:radar}
\end{subfigure}%
\hfill
\begin{subfigure}[c]{0.56\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sections/figures/semantic.pdf}
    \caption{Semantic grouping of Fused \nameofmethod{} features under speckle noise (severity 3 and 5). StableVLA preserves object-centric clusters while baselines degrade.}
    \label{fig:semantic}
\end{subfigure}
\caption{\textbf{Robustness analysis.} (a) Radar charts showing per-corruption robustness across four LIBERO task suites. StableVLA consistently outperforms baselines. (b) K-means clustering ($K\!=\!2$) of output features: standard MLP produces diffused features, while Fused \nameofmethod{} maintains coherent semantic grouping under noise.}
\label{fig:robustness_analysis}
\end{figure}

==> sections/tables/tab_main_results.tex <==
% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{3.5pt}  % 保持列间距不变，避免表格过宽
% \caption{Full comparison on LIBERO and CALVIN benchmark. Methods are grouped by training paradigm. We report success rate (\%). \textbf{Bold}: best, \underline{underline}: second best.}
% \label{tab:app_full_libero_calvin}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ll cccc cccc cccc cccc cccc}
% \toprule
%  & & \multicolumn{4}{c}{Spatial} & \multicolumn{4}{c}{Object} & \multicolumn{4}{c}{Goal} & \multicolumn{4}{c}{Long} & \multicolumn{4}{c}{CALVIN} \\  % 新增 CALVIN 列组
% \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18} \cmidrule(lr){19-22}  % 新增 CALVIN 对应的分隔线
% Training & Method & C & S3 & S4 & S5 & C & S3 & S4 & S5 & C & S3 & S4 & S5 & C & S3 & S4 & S5 & C & S3 & S4 & S5 \\  % 新增 CALVIN 的 C/S3/S4/S5 列
% \midrule
% \multirow{2}{1.2cm}{OpenX\\Pretrain} & OpenVLA (7B) & 80.0 & 40.9 & 24.6 & 14.7 & 69.6 & 18.2 & 10.4 & 2.7 & 74.0 & 38.7 & 27.0 & 16.3 & 55.5 & 20.5 & 12.4 & 7.0 & \textit{--} & \textit{--} & \textit{--} & \textit{--} \\  % 新增 CALVIN 列数据（无数据用 -- 占位）
%  & OpenVLA-OFT (7B)& 92.6 & 89.3 & \underline{84.0} & \underline{72.1} & 98.4 & 82.5 & 69.2 & 52.8 & 96.8 & \textbf{94.5} & \underline{84.6} & \underline{70.3} & \textbf{94.4} & \textbf{77.6} & 61.9 & 40.3 & \textit{--} & \textit{--} & \textit{--} & \textit{--} \\
% \midrule
% \multirow{1}{1.2cm}[8pt]{OpenX+Web\\Co-train} & 
% \rule[-10pt]{0pt}{24pt} OpenPi$\text{--}$0.5 (3B)& \textbf{98.4} & 88.3 & 79.0 & 62.4 & \textbf{99.4} & \textbf{97.1} & \textbf{88.4} & \textbf{76.4} & 97.2 & 87.2 & 82.5 & 64.2 & 92.0 & 76.1 & \textbf{65.6} & \textbf{47.7} & \textit{--} & \textit{--} & \textit{--} & \textit{--} \\
% \midrule
% \multirow{2}{1.2cm}{VLM\\Direct FT} & VLA-Adapter (0.5B)& 96.0 & \underline{93.7} & 83.3 & 58.5 & 96.8 & 71.0 & 44.1 & 29.3 & \underline{97.4} & 79.5 & 64.7 & 47.3 & \underline{94.4} & 63.5 & 41.0 & 26.2 & 4.14 & 2.56 & 1.89 & 1.44 \\
%  & StableVLA (0.5B)& \underline{96.2} & \textbf{94.3} & \textbf{92.1} & \textbf{82.0} & \underline{98.8} & \underline{92.4} & \underline{83.6} & \underline{70.2} & \textbf{98.0} & \underline{93.4} & \textbf{85.0} & \textbf{71.9} & 93.6 & \underline{76.3} & \underline{62.4} & \underline{45.3} & \textbf{4.17} & \textbf{2.77} & \textbf{2.11} & \textbf{1.51} \\  % 所有行均新增 CALVIN 列占位
% \bottomrule
% \end{tabular}}
% \end{table}

\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Full comparison on LIBERO and CALVIN benchmark. Methods are grouped by training paradigm. We report success rate (\%). \textbf{Bold}: best, \underline{underline}: second best.}
\label{tab:app_full_libero_calvin}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll cccc cccc cccc cccc cccc}
\toprule
\multirow{3}{*}{\makecell[l]{Training\\Method}} & \multirow{3}{*}{\makecell[l]{Method}} & \multicolumn{4}{c}{Spatial} & \multicolumn{4}{c}{Object} & \multicolumn{4}{c}{Goal} & \multicolumn{4}{c}{Long} & \multicolumn{4}{c}{CALVIN} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18} \cmidrule(lr){19-22}
 & & C & S3 & S4 & S5 & C & S3 & S4 & S5 & C & S3 & S4 & S5 & C & S3 & S4 & S5 & C & S3 & S4 & S5 \\
\midrule
\multirow{2}{*}{\makecell[l]{OpenX\\Pretrain}} & OpenVLA (7B) & 80.0 & 40.9 & 24.6 & 14.7 & 69.6 & 18.2 & 10.4 & 2.7 & 74.0 & 38.7 & 27.0 & 16.3 & 55.5 & 20.5 & 12.4 & 7.0 & -- & -- & -- & -- \\
 & OpenVLA-OFT (7B) & 92.6 & 89.3 & \underline{84.0} & \underline{72.1} & 98.4 & 82.5 & 69.2 & 52.8 & 96.8 & \textbf{94.5} & \underline{84.6} & \underline{70.3} & \textbf{94.4} & \textbf{77.6} & 61.9 & 40.3 & -- & -- & -- & -- \\
\midrule
\makecell[l]{OpenX+Web\\Co-train} & OpenPi--0.5 (3B) & \textbf{98.4} & 88.3 & 79.0 & 62.4 & \textbf{99.4} & \textbf{97.1} & \textbf{88.4} & \textbf{76.4} & 97.2 & 87.2 & 82.5 & 64.2 & 92.0 & 76.1 & \textbf{65.6} & \textbf{47.7} & -- & -- & -- & -- \\
\midrule
\multirow{2}{*}{\makecell[l]{VLM\\Direct FT}} & VLA-Adapter (0.5B) & 96.0 & \underline{93.7} & 83.3 & 58.5 & 96.8 & 71.0 & 44.1 & 29.3 & \underline{97.4} & 79.5 & 64.7 & 47.3 & \underline{94.4} & 63.5 & 41.0 & 26.2 & 4.14 & 2.56 & 1.89 & 1.44 \\
 & StableVLA (0.5B) & \underline{96.2} & \textbf{94.4} & \textbf{92.1} & \textbf{82.0} & \underline{98.8} & \underline{92.4} & \underline{83.6} & \underline{70.2} & \textbf{98.0} & \underline{93.4} & \textbf{85.0} & \textbf{71.9} & 93.6 & \underline{76.3} & \underline{62.4} & \underline{45.3} & \textbf{4.17} & \textbf{2.77} & \textbf{2.11} & \textbf{1.51} \\
\bottomrule
\end{tabular}}
\end{table}

% \begin{table}[t]
% \centering
% \begin{minipage}{0.6\textwidth}
%     \centering
%     \setlength{\tabcolsep}{6pt}
%     \caption{Detailed comparison between VLA-Adapter-Pro and StableVLA on LIBERO and CALVIN benchmarks. We use the latest released checkpoint for evaluation. We use success rate (ranging from 0 to 100\%) and average completed tasks (ranging from 0 to 5) as the metric for LIBERO and CALVIN, respectively. At each severity level, we report the corresponding metric averaged over all types of corruptions. The best results are highlighted in \textbf{bold}.}
%     \label{tab:detailed}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llcccccc}
%     \toprule
%     Benchmark & Task & Method & Clean & Sev 3 & Sev 4 & Sev 5 & Avg \\
%     \midrule
% \multirow{8}{*}{LIBERO} & \multirow{2}{*}{Spatial} & VLA-Adapter-Pro & 96.0 & 93.7 & 83.3 & 58.5 & 78.5 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{96.2} & \textbf{94.3} & \textbf{92.1} & \textbf{82.0} & \textbf{89.5} \\
% \cmidrule{2-8}
%  & \multirow{2}{*}{Object} & VLA-Adapter-Pro & 96.8 & 71.0 & 44.1 & 29.3 & 48.1 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{98.8} & \textbf{92.4} & \textbf{83.6} & \textbf{70.2} & \textbf{82.1} \\
% \cmidrule{2-8}
%  & \multirow{2}{*}{Goal} & VLA-Adapter-Pro & 97.4 & 79.5 & 64.7 & 47.3 & 63.8 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{98.0} & \textbf{93.4} & \textbf{85.0} & \textbf{71.9} & \textbf{83.4} \\
% \cmidrule{2-8}
%  & \multirow{2}{*}{Long} & VLA-Adapter-Pro & \textbf{94.4} & 63.5 & 41.0 & 26.2 & 43.6 \\
%  & & \textbf{StableVLA (Ours)} & 93.6 & \textbf{76.3} & \textbf{62.4} & \textbf{45.3} & \textbf{61.3} \\
% \midrule
% \multirow{2}{*}{CALVIN} & \multirow{2}{*}{-} & VLA-Adapter-Pro & 4.14 & 2.56 & 1.89 & 1.44 & 1.96 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{4.17} & \textbf{2.77} & \textbf{2.11} & \textbf{1.51} & \textbf{2.13} \\
% \bottomrule
%     \end{tabular}}
% \end{minipage}%
% \hfill
% \begin{minipage}{0.37\textwidth}
%     \centering
%     \includegraphics[width=0.95\textwidth]{sections/figures/radar_4tasks_with_clean.pdf}
%     \vspace{-0.2cm}
%     \captionof{figure}{Robustness comparison across visual corruption types on LIBERO. Each axis represents a corruption type. See Appendix~\ref{app:radar} for details.}
%     \label{fig:radar}
%     % \vspace{0.5cm}
    
%     % \includegraphics[width=\textwidth]{sections/figures/catastrophic.pdf}
%     % \vspace{-0.3cm}
%     % \caption{\textbf{Preventing Catastrophic Failure.} Under extreme corruption (Severity 5), the baseline collapses while StableVLA retains high operability.}
%     % \label{fig:failure}
% \end{minipage}
% \vspace{-10pt}
% \end{table}

% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{8pt}
% \caption{Detailed comparison between VLA-Adapter-Pro and StableVLA on LIBERO and CALVIN benchmarks. LIBERO reports success rate (\%), CALVIN reports average completed tasks (max 5). All corruption results evaluated at severity levels 3, 4, and 5.}
% \label{tab:detailed}
% \begin{tabular}{llllccccc}
% \toprule
% Benchmark & Task Suite & Method & Clean & Sev 3 & Sev 4 & Sev 5 & Avg \\
% \midrule
% \multirow{8}{*}{LIBERO} & \multirow{2}{*}{Spatial} & VLA-Adapter-Pro & 96.0 & 93.7 & 83.3 & 58.5 & 78.5 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{96.2} & \textbf{94.3} & \textbf{92.1} & \textbf{82.0} & \textbf{89.5} \\
% \cmidrule{2-8}
%  & \multirow{2}{*}{Object} & VLA-Adapter-Pro & 96.8 & 71.0 & 44.1 & 29.3 & 48.1 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{98.8} & \textbf{92.4} & \textbf{83.6} & \textbf{70.2} & \textbf{82.1} \\
% \cmidrule{2-8}
%  & \multirow{2}{*}{Goal} & VLA-Adapter-Pro & 97.4 & 79.5 & 64.7 & 47.3 & 63.8 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{98.0} & \textbf{93.4} & \textbf{85.0} & \textbf{71.9} & \textbf{83.4} \\
% \cmidrule{2-8}
%  & \multirow{2}{*}{Long} & VLA-Adapter-Pro & \textbf{94.4} & 66.7 & 43.4 & 27.6 & 45.9 \\
%  & & \textbf{StableVLA (Ours)} & 93.6 & \textbf{78.6} & \textbf{65.1} & \textbf{47.3} & \textbf{63.7} \\
% \midrule
% \multirow{2}{*}{CALVIN} & \multirow{2}{*}{-} & VLA-Adapter-Pro & 4.14 & 2.56 & 1.89 & 1.44 & 1.96 \\
%  & & \textbf{StableVLA (Ours)} & \textbf{4.17} & \textbf{2.77} & \textbf{2.11} & \textbf{1.51} & \textbf{2.13} \\
% \bottomrule
% \end{tabular}
% \end{table}
% \input{sections/tables/tab_main_results}    
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{sections/figures/libero_radar.pdf}
%     \vspace{-0.2cm}
%     \caption{\textbf{Robustness Profile (Severity 5).} Comparison across four task suites (Object, Spatial, Goal, Long). StableVLA (Blue) consistently envelopes the Baseline (Red) across all corruption categories (Noise, Blur, Weather, Digital), indicating comprehensive robustness.}
%     \label{fig:radar}
% \end{figure}
